PrO Filtering via Kernel Mean Embedding Dynamics

Filtering methods are routinely deployed with misspecified state-space models, where Bayesian filters can diverge and become overconfident. Predictively-oriented (PrO) filtering is a recent, hyperparameter-free alternative that was demonstrated to outperform (generalised) Bayesian filtering methods when either the dynamical model or the measurement model is structurally misspecified. This can be attributed to \emph{hedging} behaviour: when an observation conflicts with the forecast, the PrO update places mass near both. Yet existing implementations of PrO filtering rely on unimodal (Gaussian) approximations, whose ability to effectively hedge is limited. This paper develops the first nonparametric, particle-based implementation of PrO filtering. The key obstacle, that PrO filtering distributions are only implicitly defined, is overcome by constructing a path from the predictive to the PrO filtering distribution whose rate is available in closed form, enabling the use of kernel mean embedding dynamics for measure transport. The resulting algorithm requires only simulation from the dynamical model and evaluations of the likelihood, with neither importance weights nor the predictive density. Moreover, as we prove, the number of pseudo-time steps it requires does not grow with the outlyingness of the observation, in contrast to transport along the Bayesian tempering path. An empirical assessment shows substantial improvement over Gaussian variation of PrO filtering in challenging nonlinear examples where Gaussian approximation is unreasonably limited.

==> preamble.tex <==
%
\usepackage{acro}
\makeatletter
\@ifpackageloaded{graphicx}{}{\usepackage{graphicx}}
\@ifpackageloaded{booktabs}{}{\usepackage{booktabs}}
\@ifpackageloaded{float}{}{\usepackage{float}}
\makeatother

%
%
\providecommand{\figdir}{figs-ICML}
\graphicspath{{\figdir/}}
\ifcsname ifarxiv\endcsname\else\expandafter\newif\csname ifarxiv\endcsname\fi
%
%
\makeatletter
\@ifpackageloaded{algorithm2e}{\newcommand{\algoenv}{algorithm}}{%
  \@ifpackageloaded{algorithm}%
    {\usepackage[algo2e,ruled,vlined]{algorithm2e}\newcommand{\algoenv}{algorithm2e}}%
    {\usepackage[ruled,vlined]{algorithm2e}\newcommand{\algoenv}{algorithm}}}
\makeatother

%
\ifcsname assumption\endcsname\else\newtheorem{assumption}{Assumption}\fi
\ifcsname definition\endcsname\else\newtheorem{definition}{Definition}\fi
\ifcsname lemma\endcsname\else\newtheorem{lemma}{Lemma}\fi
\ifcsname proposition\endcsname\else\newtheorem{proposition}{Proposition}\fi
\ifcsname theorem\endcsname\else\newtheorem{theorem}{Theorem}\fi
\ifcsname remark\endcsname\else\newtheorem{remark}{Remark}\fi
\ifcsname corollary\endcsname\else\newtheorem{corollary}{Corollary}\fi

%
\newcommand{\KGD}{\mathrm{KGD}}
\newcommand{\KLD}{\mathrm{KLD}}
\newcommand{\vargrad}{\nabla_{\mathrm{V}}}
\newcommand{\dd}{\mathrm{d}}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Hk}{\mathcal{H}_k}
\newcommand{\1}{\mathbf{1}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\note}[1]{\textcolor{magenta}{[Draft note: #1]}}
\newcommand{\nik}[1]{%
    \textcolor{red}{\textbf{Nik:} #1}%
  }

%
\DeclareAcronym{kgd}{short = KGD, long = kernel gradient discrepancy}
\DeclareAcronym{kld}{short = KLD, long = Kullback--Leibler divergence}
\DeclareAcronym{mcmc}{short = MCMC, long = Markov chain Monte Carlo}
\DeclareAcronym{mmd}{short = MMD, long = maximum mean discrepancy}
\DeclareAcronym{rkhs}{short = RKHS, long = reproducing kernel Hilbert space}
\DeclareAcronym{mfld}{short = MFLD, long = mean field Langevin dynamics}
\DeclareAcronym{ula}{short = ULA, long = unadjusted Langevin algorithm}
\DeclareAcronym{sde}{short = SDE, long = stochastic differential equation}
\DeclareAcronym{PrO}{short = PrO, long = predictively oriented}
\DeclareAcronym{ode}{short = ODE, long = ordinary differential equation}

%
\makeatletter
\@ifpackageloaded{cleveref}{}{\usepackage[capitalize,noabbrev]{cleveref}}
\makeatother
\crefname{algocf}{Algorithm}{Algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}
\Crefname{assumption}{Assumption}{Assumptions}

